How do neural networks see depth in single images?

Deep neural networks have lead to a breakthrough in depth estimation from single images. Recent work often focuses on the accuracy of the depth map, where an evaluation on a publicly available test set such as the KITTI vision benchmark is often the main result of the article. While such an evaluation shows how well neural networks can estimate depth, it does not show how they do this. To the best of our knowledge, no work currently exists that analyzes what these networks have learned. In this work we take the MonoDepth network by Godard et al. and investigate what visual cues it exploits for depth estimation. We find that the network ignores the apparent size of known obstacles in favor of their vertical position in the image. Using the vertical position requires the camera pose to be known; however we find that MonoDepth only partially corrects for changes in camera pitch and roll and that these influence the estimated depth towards obstacles. We further show that MonoDepth's use of the vertical image position allows it to estimate the distance towards arbitrary obstacles, even those not appearing in the training set, but that it requires a strong edge at the ground contact point of the object to do so. In future work we will investigate whether these observations also apply to other neural networks for monocular depth estimation.

==> context.tex <==
\section{Use of context (TODO remove)}
\begin{itemize}
    \item Section 4 looked at properties of the object: position in image and apparent size. Section 5 showed that the camera pitch is estimated (although not perfectly) and used to convert the obstacle's position into a depth estimate. (Still WIP)
    \item After correcting for the camera pose, are there other parts of the image that \emph{do not} belong to the obstacle (i.e. the context) that influence the depth estimate?
    \item Experiment:
    \begin{itemize}
        \item Paste same object at same scale and position into different images of the KITTI dataset. Compare the estimated depth between these images.
        \item Paste same object on completely unrelated background image, or vertically flipped image, or white background, or ...
        \item Paste object into image, measure if \emph{other} depths changed!
    \end{itemize} 
    \item Result: the context has only a very small influence on the estimated depth of the object. In other words, the depth towards an obstacle does not (strongly) depend on other parts of the image. (WIP)
\end{itemize}

==> futurework.tex <==
\section{Future work}
The results in this work are based on a single neural network (\monodepth) trained on only one dataset (KITTI). In future work, we plan to repeat the experiments published here with other networks for depth estimation after training on the same dataset, to see if these networks learn the same behavior.
Additionally, we plan to repeat these experiments after training on a dataset with stronger variations in camera pose to see whether the network will learn to use different depth cues or whether depth estimation will fail altogether.

==> macros.tex <==
\newcommand{\monodepth}{MonoDepth}

% Formatting
\usepackage{enumitem}
\setlist[itemize]{nosep}

\hyphenation{monodepth}

% Tables
\usepackage{booktabs}

% Important numbers
\newcommand{\ntestimages}{200}

==> other.tex <==
\section{Other observations}

\begin{itemize}
    \item Flipping image
    \begin{itemize}
        \item Show strong prior beliefs of presence of road in lower half of the image and sky in the upper half.
        \item Show that \monodepth\ uses vertical position, not \emph{optical adjacency} \cite{Epstein1966a,Bian2005}. Edit: \monodepth\ does not even recognize the 'ceiling' or cars after flipping...
        \begin{itemize}
            \item Maybe try a slightly more nuanced experiment where the ground texture is interrupted. Answer: no effect.
        \end{itemize}
    \end{itemize}
    \item In the original dataset and predicted depth maps, poles always seem to end at the horizon level instead of extending further...?
\end{itemize}
